Backstepping Temporal Difference Learning

Off-policy learning ability is an important feature of reinforcement learning (RL) for practical applications. However, even one of the most elementary RL algorithms, temporal-difference (TD) learning, is known to suffer form divergence issue when the off-policy scheme is used together with linear function approximation. To overcome the divergent behavior, several off-policy TD-learning algorithms, including gradient-TD learning (GTD), and TD-learning with correction (TDC), have been developed until now. In this work, we provide a unified view of such algorithms from a purely control-theoretic perspective, and propose a new convergent algorithm. Our method relies on the backstepping technique, which is widely used in nonlinear control theory. Finally, convergence of the proposed algorithm is experimentally verified in environments where the standard TD-learning is known to be unstable.

==> discussion/discussion.tex <==
\par
Even though there are practical results showing that TDC enjoys faster convergence than GTD2 in several simple enviromental benchmarks, GTD2 has the advantage in that since it has primal dual formulation, it can be optimized by several techniques from optimization literature. Hence, we first discuss BTD1 which encompasses GTD2. Under Random walk environment, whether the tabular feature, the dependent feature, or the inverted feature is used,  BTD1 performs best when \(\eta =0.5 \), which is better than the case when \(\eta=0\). Since \(\eta =0 \) corresponds to GTD2, as \(\eta\to 0\), the performance matches that of GTD2. In a nutshell, BTD1 works well under various choices of hyperparameters, and performs comparably to GTD2. The second algorithm, BTD2 shows faster convergence than TDRC under Random walk environment with Inverted Representation when \(\eta = 0.5 \). It performs comparable to TDRC under Baird and Boyan chain. TDRC required two hyperparameters, \( \eta\) and \( \beta\) whereas BTD2 requires only one hyperparameter selection.
\par
In this paper, we have developed a new framework to design a off-policy TD algorithm, which encompasses GTD2 and TDC. We reformulated a fixed point problem to a control design problem, which enables further analysis.The time-delayed system is one method studied in control design, and it can be incorporated to our design mechanism. Other control techniques can be applied with backstepping.


